Single use register automata for data words

Our starting point are register automata for data words, in the style of Kaminski and Francez. We study the effects of the single-use restriction, which says that a register is emptied immediately after being used. We show that under the single-use restriction, the theory of automata for data words becomes much more robust. The main results are: (a) five different machine models are equivalent as language acceptors, including one-way and two-way single-use register automata; (b) one can recover some of the algebraic theory of languages over finite alphabets, including a version of the Krohn-Rhodes Theorem; (c) there is also a robust theory of transducers, with four equivalent models, including two-way single use transducers and a variant of streaming string transducers for data words. These results are in contrast with automata for data words without the single-use restriction, where essentially all models are pairwise non-equivalent.

==> atoms.tex <==











    
    
    
        


    





==> pyramid.tex <==
\section{An example of a single-use automaton}
This section is devoted to an example of a single-use automaton, which will illustrate the models presented in the rest of the paper. 
Fix for the rest of this paper an infinite set $\atoms$, whose elements are called \emph{atoms} (or data values). We will only compare atoms with respect to equality. In this paper, we study languages and transducers where the alphabets involved are built using atoms. For example, $\atoms$ is a legitimate alphabet. 

Consider the language $L \subseteq \atoms^*$ which consists of words where at most three atoms appear. One way to recognise this language is to use a one-way automaton, which has three registers that store atoms. Initially, all three registers are empty. Whenever the automaton reads an input letter, it checks if that letter is already present in one of the registers.  If it is present, it proceeds to the next input letter. If it is not present, and some register is empty, then the input letter is loaded into the first empty register. Finally, if the input letter is not present in any of the registers, and none of the registers are empty, then the automaton rejects immediately. The automaton accepts an input string if it reaches the end of the input.

The above is an example of a register automaton~\cite{bojanczyk_slightly2018}, also known as a \emph{finite memory automaton}~\cite[Definition 1]{kaminskiFiniteMemoryAutomata1994}. The topic of this paper is a restriction on the use of registers, which is called the \emph{single-use restriction}: whenever a register is used (e.g.~compared with an input letter), then its value is destroyed. The above example is does not satisfy the single-use restriction, but below we present an automaton that recognises the same language and satisfies the single-use restriction.

The key 

==> sequential.tex <==
\section{Decomposition of single-use Mealy machines}
\label{ap:proof-of-krohn-rhodes}
In this part of the appendix, we use Split Lemma from Appendix .. to prove the Krohn-Rhodes decomposition for single-use Mealy machines from Theorem~\ref{thm:mealy-machine-krohn-rhodes}. 



We start this appendix by giving exact proofs of some claims from Section \ref{sec:su-sequential}:

In order to finish the proof of the easier bottom-up implications one just have to notice,
that all the prime functions can be computed by the appropriate models.\\

\begin{lemma}
    Every function $f$ recognised by a one-way transducer with atoms, is the following composition
    \[  (homomorphism) \circ (\textrm{Mealy}) \circ (w \mapsto w \dashv)\]
\end{lemma}
\begin{proof}
    We simulate $f : \Sigma^* \to \Gamma^*$ with a Mealy machine $f' : (\Sigma + \dashv)^* \to {(\Gamma^{\leq k})}^*$,
    where $k$ is the bound from Claim \ref{claim:stay-in-place-bound}: Instead of outputting every letter the
    Mealy machine bundles up all the letters and output them all at once, when it goes forward. To get the original
    function $f$ we compose $f$ with the end mark function (from the left) and with the flattening homomorphism
    (${(\Gamma^{\leq k})}^* \to \Gamma^*$).
\end{proof}

